Uncertainty propagation for nonlinear dynamics: A polynomial optimization approach

We use Lyapunov-like functions and convex optimization to propagate uncertainty in the initial condition of nonlinear systems governed by ordinary differential equations. We consider the full nonlinear dynamics without approximation, producing rigorous bounds on the expected future value of a quantity of interest even when only limited statistics of the initial condition (e.g., mean and variance) are known. For dynamical systems evolving in compact sets, the best upper (lower) bound coincides with the largest (smallest) expectation among all initial state distributions consistent with the known statistics. For systems governed by polynomial equations and polynomial quantities of interest, one-sided estimates on the optimal bounds can be computed using tools from polynomial optimization and semidefinite programming. Moreover, these numerical bounds provably converge to the optimal ones in the compact case. We illustrate the approach on a van der Pol oscillator and on the Lorenz system in the chaotic regime.

==> Sections/03-bounds-v2.tex <==
\section{Upper bounds on maximal expectations}
\label{ss:bounds}

We now use a version of Lyapunov analysis to derive \emph{a priori} upper bounds on the maximal expectation $p^\star$. We start with a simple observation, where $\mathbb{R}_+^m$ is the cone of $m$-dimensional vectors with nonnegative entries.

\begin{proposition}
    Suppose there exist a scalar $\alpha \in \mathbb{R}$, a vector $\boldsymbol{\beta} \in \mathbb{R}_+^m$, and a function $v \in C^1([0,T]\times \mathcal{X})$ such that
    \begin{subequations}
        \begin{align}
        \label{eqn:line-2}
        \mathcal{L} v(t,\vec{x}) &\leq 0 &&\forall(t,\vec{x}) \in [0,T] \times \mathcal{X},\\
        \objFun(\vec{x}) &\leq v(T,\vec{x})
        &&\forall \vec{x} \in \mathcal{X},
        \label{eqn:line-1}\\
        v(0,\vec{x}) &\leq \alpha + \boldsymbol{\beta} \cdot \conFun(\vec{x})
        &&\forall \vec{x} \in \mathcal{X}_0.
        \label{eqn:line-3}
        \end{align}
    \end{subequations}
    Then, for every $\mu_0\in\Prob(\mathcal{X}_0)$ satisfying~\cref{e:setup:initial-stats} there holds
        \begin{equation}
        \label{e:upper-bound}
        \E_{\mu_0}[\objFun(\vec{x}(T; \vec{x}_0))] \leq \alpha + \boldsymbol{\beta} \cdot \vec{c}.
        \end{equation}
\end{proposition}

\begin{remark}\label{r:v-nonincreasing}
    The function $v$ is not a Lyapunov function, but resembles one because, by \cref{e:lie-derivative-identity} and \cref{eqn:line-2}, it does not increase along solutions of the ODE \cref{e:ode} over the time interval $[0,T]$.
\end{remark}

\begin{proof}
%By \cref{e:lie-derivative-identity}, condition \cref{eqn:line-2} implies that the function $v$ does not increase along solutions of the ODE \cref{e:ode} over the time interval $[0,T]$. 
As noted in \cref{r:v-nonincreasing}, $v(t,\vec{x}(t;\vec{x}_0))$ does not increase over the time interval $[0,T]$. Consequently, inequalities \cref{eqn:line-1,eqn:line-3} imply that, for any initial condition $\vec{x}_0 \in \mathcal{X}_0$,
\begin{equation*}
    \objFun(\vec{x}(T; \vec{x}_0))
    \leq
    v(T, \vec{x}(T; \vec{x}_0))
    \leq
    v(0, \vec{x}_0)
    \leq
    \alpha + \boldsymbol{\beta} \cdot \conFun(\vec{x}_0).
\end{equation*}
Taking expectations with respect to the distribution $\mu_0$ of the initial condition $\vec{x}_0$ and applying \cref{e:setup:initial-stats} yields \cref{e:upper-bound}.
\end{proof}

Maximizing the left-hand side of \cref{e:upper-bound} over all probability measures $\mu_0$ consistent with \cref{e:setup:initial-stats} and minimizing the right-hand side over $\alpha$, $\boldsymbol{\beta}$ and $v$ gives our first main result.

\begin{theorem}
    There holds
    \begin{equation}\label{e:weak-duality}
        p^\star \leq \inf_{
            \substack{
                \alpha \in \mathbb{R},\,
                \boldsymbol{\beta} \in \mathbb{R}_+^m\\
                v \in C^1([0,T]\times \mathcal{X})\\
                \text{s.t. \cref{eqn:line-1,eqn:line-2,eqn:line-3}}
            }
        } \left\{\alpha + \boldsymbol{\beta}\cdot \vec{c} \right\}
        =: d^\star.
    \end{equation}
\end{theorem}

Inequality \cref{e:weak-duality} expresses the weak duality between the maximal expectation problem \cref{e:setup:max-expectation} and the minimization problem for the optimal upper bound $d^\star$. Next, we prove that if the sets $\mathcal{X}_0$ and $\mathcal{X}$ are compact this duality is in fact strong, meaning that the upper bound $d^\star$ obtained by optimizing the `auxiliary' function $v$ evaluates $p^\star$ exactly.

\begin{theorem}\label{th:strong-duality}
    If $\mathcal{X}_0$ and $\mathcal{X}$ are compact, $p^\star = d^\star$.
\end{theorem}

\begin{proof}
    Recall from \cref{prop:max-expectation-measures} that $p^\star$ is the optimal value of the linear program over measures in~\cref{e:setup:max-expectation-measures}. Let
    \begin{align*}
        \Lambda(\lambda,\mu,\nu; v,\boldsymbol{\beta}) :=
        \boldsymbol{\beta}\cdot\vec{c}%&
        +
        \int_{\mathcal{X}_0} \left[v(0,\vec{x}) - \boldsymbol{\beta} \cdot \vec{h}(\vec{x})\right] \rd\lambda(\vec{x})&
        \\
        + \int_{\mathcal{X}} \left[g(\vec{x}) - v(T,\vec{x}) \right]\rd\nu(\vec{x})&
        \\
        + \int_{[0,T]\times \mathcal{X}} \mathcal{L}v(t,\vec{x}) \, \rd\mu(t,\vec{x})&
    \end{align*}
    be the corresponding Lagrangian, where $v \in C^1([0,T]\times\mathcal{X})$ and $\beta \in \mathbb{R}^m$ are Lagrange multipliers for the constraints of~\cref{e:setup:max-expectation-measures}. Set $\Omega := [0,T]\times \mathcal{X}$. We show that
    \begin{subequations}
        \begin{align}
        \label{e:strong-duality:step1}
        p^\star
        &=
        \sup_{\substack{
            \lambda \in \Prob(\mathcal{X}_0)\\
            \nu \in \Prob(\mathcal{X})\\
            \mu \in T\Prob(\Omega)
        }}
        \inf_{\substack{
            \boldsymbol{\beta} \in \mathbb{R}_+^m\\
            v \in C^1(\Omega)
        }}
        \Lambda(\lambda,\mu,\nu; v,\boldsymbol{\beta})
        \\
        \label{e:strong-duality:step2}
        &=
        \inf_{\substack{
            \boldsymbol{\beta} \in \mathbb{R}_+^m\\
            v \in C^1(\Omega)
        }}
        \sup_{\substack{
            \lambda \in \Prob(\mathcal{X}_0)\\
            \nu \in \Prob(\mathcal{X})\\
            \mu \in T\Prob(\Omega)
        }}
        \Lambda(\lambda,\mu,\nu; v,\boldsymbol{\beta})
        \\
        \label{e:strong-duality:step3}
        &= d^\star.
    \end{align}
    \end{subequations}
    The equality in~\cref{e:strong-duality:step1} holds because the inner infimum is unbounded below unless $\lambda$, $\nu$ and $\mu$ satisfy the constraints of~\cref{e:setup:max-expectation-measures}. 
    % For the second equality, observe that since $\mathcal{X}$ and $\mathcal{X}_0$ are compact, the set $\mathbb{X} = \Prob(\mathcal{X}_0) \times \Prob(\mathcal{X}) \times T\Prob(\Omega)$ equipped with the product weak-star topology is a compact convex subset of a linear topological space. Similarly, $\mathbb{Y} = \mathbb{R}^m_+ \times C^1(\Omega)$ in the usual product topology is a convex subset of a linear space. The Lagrangian $\Lambda$ is both linear and continuous on $\mathbb{X} \times \mathbb{Y}$ for the stated topologies, so a minimax theorem due to Sion \cite{Sion1958} (see also the introduction of \cite{Komiya1988}), which states that the order of inf and sup can be reversed without introducing a duality gap.
    The equality in~\cref{e:strong-duality:step2} follows from a minimax theorem due to Sion \cite{Sion1958} (see also \cite{Komiya1988}), which states that the order of inf and sup can be reversed without introducing a duality gap. To use this theorem, recall that
    $\mathcal{X}$ and $\mathcal{X}_0$ are compact, so $\mathbb{X} = \Prob(\mathcal{X}_0) \times \Prob(\mathcal{X}) \times T\Prob(\Omega)$ equipped with the product weak-star topology is a compact convex subset of a linear topological space. Observe also that
    $\mathbb{Y} = \mathbb{R}^m_+ \times C^1(\Omega)$ with the usual product topology is a convex subset of a linear space.
    Finally, note that the Lagrangian $\Lambda$ is linear and continuous on $\mathbb{X} \times \mathbb{Y}$ for the stated topologies. We have thus verified all assumptions of Sion's theorem.

    We now turn to the equality in~\cref{e:strong-duality:step3}. The inner maximum over $\lambda$, $\nu$ and $\mu$ in~\cref{e:strong-duality:step2} is attained by Dirac measures at the maximizers of $v(0,\cdot) -\boldsymbol{\beta} \cdot \vec{h}(\cdot)$, $g(\cdot) - v(T,\cdot)$ and $\mathcal{L}v$, respectively. Thus,
    \begin{align*}
        p^\star =
        \inf_{\substack{
            \boldsymbol{\beta} \in \mathbb{R}_+^m\\
            v \in C^1(\Omega)
        }}
        \big\{
            \boldsymbol{\beta}\cdot\vec{c} +
            \max_{\vec{x} \in \mathcal{X}_0} \left[v(0,\vec{x}) - \boldsymbol{\beta} \cdot \vec{h}(\vec{x})\right]&
            \\[-2.5ex]
            + \max_{\vec{x} \in \mathcal{X}} \left[g(\vec{x}) - v(T,\vec{x})\right]&
            \\
            + T \max_{(t,\vec{x}) \in \Omega} \mathcal{L}v(t,\vec{x})&
        \big\}.
    \end{align*}
    The right-hand infimum is unchanged if $v$ is replaced with
    \begin{multline*}
        v'(t,\vec{x}) := v(t,\vec{x})
        + \max_{\vec{x} \in \mathcal{X}} \left[g(\vec{x}) - v(T,\vec{x})\right]
        \\
        + (T-t) \max_{(t,\vec{x}) \in \Omega} \mathcal{L}v(t,\vec{x}),
    \end{multline*}
    which satisfies \cref{eqn:line-1,eqn:line-2}. Consequently,
    \begin{equation*}
        p^\star = \inf_{\substack{
            \boldsymbol{\beta} \in \mathbb{R}_+^m,\,
            v \in C^1(\Omega)\\
            \text{s.t. \cref{eqn:line-1,eqn:line-2}}
        }}
            \big\{
            \boldsymbol{\beta}\cdot\vec{c} + \max_{\vec{x} \in \mathcal{X}_0} \left[v(0,\vec{x}) - \boldsymbol{\beta} \cdot \vec{h}(\vec{x})\right]
            \big\}
    \end{equation*}
    and the right-hand side is clearly equal to $d^\star$.
\end{proof}

